Temporal FiLM: Capturing Long-Range Sequence Dependencies with Feature-Wise Modulations

Learning representations that accurately capture long-range dependencies in sequential inputs -- including text, audio, and genomic data -- is a key problem in deep learning. Feed-forward convolutional models capture only feature interactions within finite receptive fields while recurrent architectures can be slow and difficult to train due to vanishing gradients. Here, we propose Temporal Feature-Wise Linear Modulation (TFiLM) -- a novel architectural component inspired by adaptive batch normalization and its extensions -- that uses a recurrent neural network to alter the activations of a convolutional model. This approach expands the receptive field of convolutional sequence models with minimal computational overhead. Empirically, we find that TFiLM significantly improves the learning speed and accuracy of feed-forward neural networks on a range of generative and discriminative learning tasks, including text classification and audio super-resolution

==> figures/Makefile <==
all:

spectrogram.png:
	python ./specfig.py \
		../../../p225_365.wav.l2-b8-reload-l2.audioresnet.multispeaker.128-128.9-9.4.1.0-0.0.relu-2-2.hr.wav \
		../../../p225_365.wav.l2-b8-reload-l2.audioresnet.multispeaker.128-128.9-9.4.1.0-0.0.relu-2-2.lr.wav \
		../../../p225_365.wav.l2-b8-reload-l2.audioresnet.multispeaker.128-128.9-9.4.1.0-0.0.relu-2-2.pr.wav

